DQNC2S: DQN-based Cross-stream Crisis event Summarizer

Summarizing multiple disaster-relevant data streams simultaneously is particularly challenging as existing Retrieve&Re-ranking strategies suffer from the inherent redundancy of multi-stream data and limited scalability in a multi-query setting. This work proposes an online approach to crisis timeline generation based on weak annotation with Deep Q-Networks. It selects on-the-fly the relevant pieces of text without requiring neither human annotations nor content re-ranking. This makes the inference time independent of the number of input queries. The proposed approach also incorporates a redundancy filter into the reward function to effectively handle cross-stream content overlaps. The achieved ROUGE and BERTScore results are superior to those of best-performing models on the CrisisFACTS 2022 benchmark.

==> tables/results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\cmidrule(l){2-7}
      & \multicolumn{2}{c|}{ICS} & \multicolumn{2}{c|}{Wikipedia} & \multicolumn{2}{c}{NIST} \\ \midrule
Event & BERT-Score   & ROUGE-2   & BERT-Score      & ROUGE-2      & BERT-Score   & ROUGE-2   \\ \midrule
001   & 0,5490       & 0,0990    & 0,5920          & 0,0223       & 0,5720       & 0,2337    \\
002   & 0,5350       & 0,0514    & 0,5901          & 0,0479       & 0,5479       & 0,0535    \\
003   & 0,5413       & 0,0583    & 0,6044          & 0,0216       & 0,6051       & 0,2420    \\
004   & 0,4797       & 0,0579    & 0,5474          & 0,0586       & 0,5337       & 0,2011    \\
005   & -            & -         & 0,5617          & 0,0479       & 0,6320       & 0,1558    \\
006   & 0,5087       & 0,0509    & 0,5567          & 0,0250       & 0,5243       & 0,0561    \\
007   & 0,5157       & 0,0295    & 0,5646          & 0,0771       & 0,5591       & 0,0916    \\
008   & 0,5178       & 0,0149    & 0,5491          & 0,0355       & 0,5927       & 0,1785    \\ \midrule
Mean  & 0,4559       & 0,0452    & 0,5707          & 0,0420       & 0,5709        & 0,1515   \\ \bottomrule
\end{tabular}

==> tables/results_no_cluster.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\cmidrule(l){2-7}
      & \multicolumn{2}{c|}{ICS} & \multicolumn{2}{c|}{Wikipedia} & \multicolumn{2}{c}{NIST} \\ \midrule
Event & BERT-Score   & Rouge-2   & BERT-Score      & Rouge-2      & BERT-Score   & Rouge-2   \\ \midrule
001   & 0,5331       & 0,1084    & 0,5518          & 0,0169       & 0,5512       & 0,2603    \\
002   & 0,5490       & 0,0310    & 0,5739          & 0,0517       & 0,5698       & 0,0554    \\
003   & 0,5375       & 0,0538    & 0,5927          & 0,0215       & 0,6197       & 0,2606    \\
004   & 0,4923       & 0,0448    & 0,5365          & 0,0644       & 0,5265       & 0,1862    \\
005   & -            & -         & 0,5643          & 0,0335       & 0,6200       & 0,1735    \\
006   & 0,5179       & 0,0370    & 0,5170          & 0,0249       & 0,5201       & 0,0370    \\
007   & 0,5391       & 0,0396    & 0,5761          & 0,0605       & 0,5595       & 0,0889    \\
008   & 0,5078       & 0,0153    & 0,5177          & 0,0418       & 0,5976       & 0,1681    \\ \midrule
Mean  & 0,4596       & 0,0412    & 0,5538          & 0,0394       & 0,5706       & 0,1538   
\end{tabular}
